Data Augmentation on Graphs: A Technical Survey

In recent years, graph representation learning has achieved remarkable success while suffering from low-quality data problems. As a mature technology to improve data quality in computer vision, data augmentation has also attracted increasing attention in graph domain. To advance research in this emerging direction, this survey provides a comprehensive review and summary of existing graph data augmentation (GDAug) techniques. Specifically, this survey first provides an overview of various feasible taxonomies and categorizes existing GDAug studies based on multi-scale graph elements. Subsequently, for each type of GDAug technique, this survey formalizes standardized technical definition, discuss the technical details, and provide schematic illustration. The survey also reviews domain-specific graph data augmentation techniques, including those for heterogeneous graphs, temporal graphs, spatio-temporal graphs, and hypergraphs. In addition, this survey provides a summary of available evaluation metrics and design guidelines for graph data augmentation. Lastly, it outlines the applications of GDAug at both the data and model levels, discusses open issues in the field, and looks forward to future directions. The latest advances in GDAug are summarized in GitHub.

==> 123.tex <==
\begin{table}
    \renewcommand\arraystretch{1}
    \centering
    \caption{Summary of representative graph data augmentation works for graph learning.}
    \label{tb: all-work}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccll}
    \toprule
    Ref              & Publication   & Year & GDAug                                   & Code                                                                                                      \\
    \midrule
    DGI              & ICLR          & 2019 & FS, ER                                  & https://github.com/PetarV-/DGI                                                                                                \\
    \midrule
    STDGI            & ICLR-workshop & 2019 & FS                                      & ---                                                                                                                          \\
    \midrule
    STABLE           & KDD           & 2022 & FS, ER                                  & ---                                                                                                                          \\
    \midrule
    HDMI             & WWW           & 2021 & FS                                      & https://github.com/baoyujing/HDMI                                                                                             \\
    \midrule
    HDGI             & AAAI-workshop & 2020 & FS                                      & https://github.com/YuxiangRen/Heterogeneous-Deep-Graph-Infomax                                                                \\
    \midrule
    HTC              & Arxiv         & 2021 & FS                                      & ---                                                                                                                          \\
    \midrule
    Contrast-Reg     & Arxiv         & 2021 & FS                                      & ---                                                                                                                          \\
    \midrule
    FLAG             & CVPR          & 2022 & FM                                      & https://github.com/devnkong/FLAG                                                              \\
    \midrule
    Ethident         & IEEE-TIFS     & 2022 & FM, ND, ER, SSa                         & https://github.com/jjzhou012/Ethident                                                         \\
    \midrule                       
    SMICLR           & JCIM          & 2022 & FM, ND, ER, SSa                         & https://github.com/CIDAG/SMICLR                                                               \\
    \midrule                       
    GraphCL          & NeurIPS       & 2020 & FM, ND, ER, SSa                         & https://github.com/Shen-Lab/GraphCL                                                           \\
    \midrule                       
    JOAO             & ICML          & 2021 & FM, ND, ER, SSa                         & https://github.com/Shen-Lab/GraphCL\_Automated                                                \\
    \midrule                       
    AutoGRL          & IJCNN         & 2021 & FM, ND, ER, PL                          & https://github.com/JunweiSUN/AutoGRL                                                          \\
    \midrule
    LG2AR            & arXiv         & 2022 & FM, ND, ER, SSa                         & ---                                                                                                                          \\
    \midrule
    GRACE            & ICML-workshop & 2020 & FM, ER                                  & https://github.com/CRIPAC-DIG/GRACE                                                           \\
    \midrule
    GCA              & WWW           & 2021 & FM, ER                                  & https://github.com/CRIPAC-DIG/GCA                                                             \\
    \midrule
    BGRL             & ICLR-workshop & 2021 & FM, ER                                  & https://github.com/nerdslab/bgrl                                                              \\
    \midrule
    BGRL             & ICLR          & 2022 & FM, ER                                  & https://github.com/Namkyeong/BGRL\_Pytorch                                                    \\
    \midrule
    GROC             & WWW-workshop  & 2021 & FM, ER                                  & ---                                                                                                                          \\
    \midrule
    GBT              & KBS           & 2022 & FM, ER                                  & https://github.com/pbielak/graph-barlow-twins                                                 \\
    \midrule
    NodeAug          & KDD           & 2020 & FM, ER                                  & ---                                                                                                                          \\
    \midrule
    MeTA             & NeurIPS       & 2021 & FM, ER                                  & ---                                                                                                                          \\
    \midrule
    MERIT            & IJCAI         & 2021 & FM, ER, GP                              & https://github.com/GRAND-Lab/MERIT                                                            \\
    \midrule
    HeCo             & KDD           & 2021 & ND                                      & https://github.com/liun-online/HeCo                                                           \\
    \midrule
    GRAND            & NeurIPS       & 2020 & ND                                      & https://github.com/THUDM/GRAND                                                                \\
    \midrule
    MH-Aug           & NeurIPS       & 2021 & ND, ER                                  & https://github.com/hyeonzini/Metropolis-Hastings-Data-Augmentation-for-Graph-Neural-Networks  \\
    \midrule
    CSSL             & AAAI          & 2021 & ND, ER                                  & https://github.com/UCSD-AI4H/GraphSSL                                                         \\
    \midrule
    two-branch Mixup & WWW           & 2021 & NI, GI                                  & https://github.com/vanoracai/MixupForGraph                                                    \\
    \midrule
    GraphMix         & AAAI          & 2021 & NI                                      & https://github.com/vikasverma1077/GraphMix                                                    \\
    \midrule
    GraphSMOTE       & WSDM          & 2021 & NI                                      & https://github.com/TianxiangZhao/GraphSmote                                                   \\
    \midrule
    GraphENS         & AAAI          & 2022 & NI                                      & https://github.com/JoonHyung-Park/GraphENS                                                    \\
    \midrule
    NodeAug-INS      & CDS           & 2021 & NI                                      & ---                                                                                                                              \\
    \midrule
    GraphMixup       & ECML-PKDD     & 2021 & NI                                      & https://github.com/LirongWu/GraphMixup                                                        \\
    \midrule
    AugAN            & arXiv         & 2022 & NI                                      & ---                                                                                                                          \\
    \midrule
    DropEdge         & ICLR          & 2020 & ER                                      & https://github.com/DropEdge/DropEdge                                                                                          \\
    \midrule
    GAUG             & AAAI          & 2021 & ER                                      & https://github.com/zhao-tong/GAug                                                                                             \\
    \midrule
    RobustECD        & IEEE-TKDE     & 2021 & ER                                      & https://github.com/jjzhou012/RobustECD                                                                                        \\
    \midrule
    FairDrop         & IEEE TAI      & 2021 & ER                                      & https://github.com/ispamm/FairDrop                                                                                            \\
    \midrule
    RT-GCN           & KDD           & 2022 & ER                                      & ---                                                                                                                          \\
    \midrule
    BiGI             & WSDM          & 2021 & ER                                      & https://github.com/caojiangxia/BiGI                                                                                           \\
    \midrule
    AD-GCL           & NeurIPS       & 2021 & ER                                      & https://github.com/susheels/adgcl                                                                                             \\
    \midrule
    AdaEdge          & AAAI          & 2020 & ER                                      & https://github.com/victorchen96/MadGap                                                                                        \\
    \midrule
    PTDNet           & WSDM          & 2021 & ER                                      & https://github.com/flyingdoog/PTDNet                                                                                          \\
    \midrule
    M-Evolve         & IEEE-TNSE     & 2020 & ER, PL                                  & ---                                                                                                                              \\
    \midrule
    SUGAR            & WWW           & 2021 & SSa                                     & https://github.com/RingBDStack/SUGAR                                                          \\
    \midrule
    GCC              & KDD           & 2020 & SSa                                     & https://github.com/THUDM/GCC                                                                  \\
    \midrule
    SUBG-COM         & ICDM          & 2020 & SSa                                     & https://github.com/yzjiao/Subg-Con                                                            \\
    \midrule
    GraphCrop        & arXiv         & 2020 & SSa                                     & ---                                                                                                 \\
    \midrule
    InfoGraph        & ICLR          & 2020 & SSa                                     & https://github.com/fanyun-sun/InfoGraph                                                       \\
    \midrule
    EGI              & NeurIPS       & 2021 & SSa                                     & https://github.com/GentleZhu/EGI                                                              \\
    \midrule
    NeuralSparse     & ICML          & 2020 & SSa                                     & https://github.com/flyingdoog/PTDNet/tree/main/NeuralSparse                                   \\
    \midrule
    MVGRL            & ICML          & 2020 & SSa, GP                                 & https://github.com/kavehhassani/mvgrl                                                                                         \\
    \midrule
    SubMix           & WWW           & 2022 & SSu                                     & https://github.com/snudatalab/GraphAug                                                                                        \\
    \midrule
    Graph Transplant & AAAI          & 2022 & SSu                                     & ---                                                                                                                          \\
    \midrule
    MoCL             & KDD           & 2021 & SSu                                     & https://github.com/illidanlab/MoCL-DK                                                         \\
    \midrule
    GREA             & KDD           & 2022 & SSu                                     & https://github.com/liugangcode/GREA                                                           \\
    \midrule
    SelfGNN          & WWW-workshop  & 2021 & GP                                      & https://github.com/zekarias-tilahun/SelfGNN                                                                                   \\
    \midrule
    MV-GCN           & CIKM          & 2021 & GP                                      & ---                                                                                                                              \\
    \midrule
    GDC              & NeurIPS       & 2019 & GP                                      & https://github.com/gasteigerjo/gdc                                                                                            \\
    \midrule
    G-mixup          & ICML          & 2022 & GI                                      & https://github.com/ahxt/g-mixup                                                               \\
    \midrule
    ifMixup          & arXiv         & 2021 & GI                                      & ---                                                                                                                              \\
    \midrule
    GraphMix         & AAAI          & 2021 & SL                                      & https://github.com/vikasverma1077/GraphMix                                                                                    \\
    \midrule
    NASA             & AAAI          & 2022 & SL                                      & https://github.com/BUPT-GAMMA/NASA                                                                                            \\
    \midrule
    CGCN             & AAAI          & 2020 & PL                                      & ---                                                                                                                          \\
    \midrule
    M3S              & AAAI          & 2020 & PL                                      & https://github.com/Junseok0207/M3S\_Pytorch                                                                                   \\
    \midrule
    NRGNN            & KDD           & 2021 & PL                                      & https://github.com/EnyanDai/NRGNN                                                                                             \\
    \bottomrule              
\end{tabular}}
\end{table}


==> 4-6-label-1.tex <==
\subsection{Label-level Augmentation}
Most of \gda~ strategies mainly manipulate the features and structure of existing graphs to achieve augmentation, without specific constraints on labels.
While label-level augmentation is another important techniques used to augment the limited labeled data using the unlabeled data.
We divide the existing label-level augmentations into pseudo-labeling and sharpening-labeling.
% 4.6.1  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Pseudo-Labeling}\label{sec: pseudo-labeling}
This strategy is generally regarded as a semi-supervised method to augment the limited labeled data by generating pseudo-labels for unlabeled data.
It is commonly used in conjunction with self-training~\cite{self-training-1,self-training-2} and co-training~\cite{co-training}.
% Here we present the following generalized definition of pseudo-labeling:
% \begin{definition}
% \begin{mydef}{~{Pseudo-Labeling}}{DEFexample}
%     % \textbf{Pseudo-Labeling}.
%     For a partially labeled dataset $\mathcal{D}=\mathcal{D}_\textit{l} \cup \mathcal{D}_\textit{u}$ that can be split into a labeled set $\mathcal{D}_\textit{l} = \left\{(\boldsymbol{x}_\textit{i}^\textit{l}, y_\textit{i}^\textit{l})\right\}_{i=1}^{|\mathcal{D}_\textit{l}|}$ and an unlabeled set $\mathcal{D}_\textit{u} = \left\{\boldsymbol{x}_\textit{i}^\textit{u}\right\}_{i=1}^{|\mathcal{D}_\textit{u}|}$, pseudo-labeling first trains a predictor using the partially labeled dataset, then generates pseudo labels for the unlabeled set, and finally filters out the pseudo labels with high confidence as the augmented labeled set $\hat{\mathcal{D}}_\textit{l}$, \ie
%     \begin{equation}
%         \begin{array}{c}
%             f: \mathcal{D} \rightarrow \mathbb{R}^\textit{c}, \quad \mathcal{Y}_\textit{u} = f(\mathcal{D}_\textit{u}) \vspace{1ex}\\
%             \mathcal{D}_\textit{p} = \operatorname{LabelFilter}(\mathcal{D}_\textit{u}, \mathcal{Y}_\textit{u}) = \left\{(\boldsymbol{x}_\textit{i}^\textit{u}, y_\textit{i}^\textit{u}) \mid \boldsymbol{x}_\textit{i}^\textit{u} \in \mathcal{D}_\textit{u}, y_\textit{i}^\textit{u} \in \mathcal{Y}_\textit{u} \right\}_{i=1}^{K} \vspace{1ex}\\
%             \hat{\mathcal{D}}_\textit{l} = \mathcal{D}_\textit{l} \cup \mathcal{D}_\textit{p}
%         \end{array}
%     \end{equation}
%     where $f$ is the pre-trained label predictor, $\mathcal{Y}_\textit{u}$ is the predictive labels of unlabeled set, $\operatorname{LabelFilter}$ is a process of filtering the pseudo labels with high confidence, $\mathcal{D}_\textit{p}$ is the retained pseudo-labeled set of size $K$ and $1 \leqslant  K  \leqslant |\mathcal{D}_\textit{u}|$.
% \end{mydef}
\begin{mydef}{~{Pseudo-Labeling}}{DEFexample}
    % The pseudo-labeling technique for a partially labeled dataset $\mathcal{D}=\mathcal{D}_\textit{l} \cup \mathcal{D}_\textit{u}$ involves initial pre-training of a predictor $f$ using the available data, followed by generation of pseudo-labels for the unlabeled samples $\mathcal{D}_\textit{u}$ using this predictor, and finally applying a labeling filter $\mathcal{F}$ to retain only those pseudo-labels with high confidence, yielding an augmented labeled set.
    % \textbf{Pseudo-Labeling}.
    For a partially labeled dataset $\mathcal{D}=\mathcal{D}_\textit{l} \cup \mathcal{D}_\textit{u}$, where $\mathcal{D}_\textit{l}$ is the labeled set and $\mathcal{D}_\textit{u}$ is the unlabeled set, the general workflow of pseudo-labeling augmentation proceeds as follows:
    \begin{enumerate}[leftmargin=18pt]
        \item pre-train a predictor $f$ using the partially labeled dataset $\mathcal{D}$;
        \item predict the pseudo-labels for the unlabeled set $\mathcal{D}_\textit{u}$ using the predictor $f$;
        \item use a labeling filter $\mathcal{F}$ to generate the augmented labeled set $\mathcal{D}_\textit{p}$ by retaining those samples with high-confidence pseudo-labels;
        \item retrain the predictor using the augmented set.
    \end{enumerate}
    The process of pseudo-labeling and model training can go through multiple rounds.
    %  first trains a predictor $f$ using the partially labeled dataset $\mathcal{D}$, then uses $f$ to generate pseudo labels for the samples in the unlabeled set, and finally filters out the pseudo labels with high confidence as the augmented labeled set $\hat{\mathcal{D}}_\textit{l}$, \ie
    % \begin{equation}
    %     \begin{array}{c}
    %         f: \mathcal{D} \rightarrow \mathbb{R}^\textit{c}, \quad \mathcal{Y}_\textit{u} = f(\mathcal{D}_\textit{u}) \vspace{1ex}\\
    %         \mathcal{D}_\textit{p} = \operatorname{LabelFilter}(\mathcal{D}_\textit{u}, \mathcal{Y}_\textit{u}) = \left\{(\boldsymbol{x}_\textit{i}^\textit{u}, y_\textit{i}^\textit{u}) \mid \boldsymbol{x}_\textit{i}^\textit{u} \in \mathcal{D}_\textit{u}, y_\textit{i}^\textit{u} \in \mathcal{Y}_\textit{u} \right\}_{i=1}^{K} \vspace{1ex}\\
    %         \hat{\mathcal{D}}_\textit{l} = \mathcal{D}_\textit{l} \cup \mathcal{D}_\textit{p}
    %     \end{array}
    % \end{equation}
    % where $f$ is the pre-trained label predictor, $\mathcal{Y}_\textit{u}$ is the predictive labels of unlabeled set, $\operatorname{LabelFilter}$ is a process of filtering the pseudo labels with high confidence, $\mathcal{D}_\textit{p}$ is the retained pseudo-labeled set of size $K$ and $1 \leqslant  K  \leqslant |\mathcal{D}_\textit{u}|$.
\end{mydef}
\begin{table*}[htp]
    \renewcommand\arraystretch{1.3}
    \centering
    \caption{Summary of different label-level augmentations.}
    \label{tb: pseudo-labeling-strategy}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccc} 
    \hline\hline
    \multirow{2}{*}{Reference} & \multirow{2}{*}{Type (custom)} & \multicolumn{2}{c}{Label-level Augmentation Setting}                                                                          \\ 
    \cline{3-4}
                                   &                   & Pseudo label generation for unlabeled data $\boldsymbol{x}^\textit{u}$               & Label filtering $\mathcal{F}$          \\ 
    \hline       
    M-Evolve~\cite{MEvolve-tnse}   & threshold-based   & same as the original graph                                                           & threshold             \\
    AutoGRL~\cite{AutoGRL-2021}    & threshold-based   & label propagation algorithm (LPA)~\cite{LPA-2003}                                    & threshold             \\
    NRGNN~\cite{NRGNN-2021}        & threshold-based   & semi-supervised prediction                                                           & threshold             \\
    CGCN~\cite{CGCN-2020}          & clustering-based  & pass the label of the labeled node to it in the same cluster	                      & match the prediction  \\
    M3S~\cite{M3S-2020}            & clustering-based  & assign the label of the nearest cluster of labeled nodes to the cluster it locates   & match the prediction  \\
    \hdashline
    GraphMix~\cite{Graphmix-2021}  & sharpening        & apply sharpening to the average predictions across multiple perturbations of it      & /                     \\
    GRAND~\cite{GRAND-2020}        & sharpening        & apply sharpening to the average predictions across multiple augmentations of it      & /                     \\
    NASA~\cite{NASA-2022}          & sharpening        & apply sharpening to the average of its neighbors' predictions                        & /                     \\
    \hline\hline
    \end{tabular}}
\end{table*}
\begin{figure*}[htp]
	\centering
		\includegraphics[width=\textwidth]{image/DA/DA_label-pseudo.pdf}
		\caption{Illustration of pseudo-labeling augmentation. The general workflow proceeds as follows: 
        1) pre-train predictor using the partially labeled dataset;
        2) predict the pseudo labels for unlabeled data using predictor;
        3) filter the pseudo labels with high confidence;
        4) retrain the predictor using the augmented set.}
		\label{fig: pseudo-labeling}
\end{figure*}
% After pseudo-labeling, the augmented set $\hat{\mathcal{D}}_\textit{l}$ can be used to retrain the predictor or train a new model.
% And the process of pseudo-labeling and model training can go through multiple rounds.
We summarize several graph related works using pseudo-labeling techniques and divide them into two categories, as listed in Table~\ref{tb: pseudo-labeling-strategy} and illustrated in Fig.~\ref{fig: pseudo-labeling}.
The \textbf{threshold-based} methods mainly construct pseudo-labels via model predictions and determine whether a pseudo-labeled sample has high confidence by comparing the model prediction probability with a threshold.
M-Evolve~\cite{MEvolve-tnse} first generates the virtual graphs via edge rewiring and assigns them the labels of the original graphs as pseudo-labels. Then a concept of label reliability is introduced based on the intuition that pseudo-labels generally have higher reliability when matched to predictions. M-Evolve finally uses the label reliability threshold to filter out the virtual graphs with high label reliability as the augmented data.
NRGNN~\cite{NRGNN-2021} first inserts the missing edges between labeled and unlabeled nodes through edge prediction, then trains a GNN model on the rewired graph and uses the predictions of unlabeled nodes as their pseudo-labels, and finally retains the unlabeled nodes with their pseudo-labels whose predicted probability is greater than a threshold as augmented data.
The \textbf{clustering-based} methods mainly use cluster assignments as pseudo-labels by introducing unsupervised clustering tasks, and then filter pseudo-labeled samples with high confidence by matching the consistency of supervised predictions and cluster assignments.
M3S~\cite{M3S-2020} first runs K-means clustering on the node embeddings, then aligns labeled and unlabeled clusters by comparing the distance of centroids between clusters, and finally passes the label of the labeled cluster to the nearest unlabeled cluster.
CGCN~\cite{CGCN-2020} first learns clusters by GMM-VGAE model, then select the highest confidence (softmax prediction score) labeled sample of each class, and finally passes their labels to the unlabeled nodes in the clustering network.

% 4.6.2  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htp]
	\centering
		\includegraphics[width=\textwidth]{image/DA/DA_label-sharpen.pdf}
		\caption{Illustration of sharpening-labeling augmentation. The general workflow proceeds as follows:
        1) pre-train predictor using the partially labeled dataset;
        2) generate $N$ augmentations of unlabeled data;
        3) generate predicted probability distributions across $N$ augmentations via predictor;
        4) compute the average prediction distribution;
        5) apply sharpening function to generate sharpened label for unlabeled data;
        6) update the predictor using the augmented set.
        } 
		\label{fig: sharpening-labeling}
\end{figure*}
\subsubsection{Sharpening-Labeling}
Pseudo-labeling techniques are obsessed with generating high-confidence pseudo-labels for unlabeled data, which usually fail when unlabeled data has low-confidence predictions. While sharpening-labeling does not rely on high-confidence predictions and is suitable for more unlabeled scenarios.
Here we present the definition of sharpening-labeling as follows:
\begin{definition}
    \textbf{Sharpening-Labeling}.
    \emph{Given predicted probability distributions $\left\{\boldsymbol{p}_\textit{i}\right\}^\textit{N}_{i=1}$ across $N$ augmentations of $\boldsymbol{x}^\textit{u}$, sharpening-labeling first computes the average prediction distribution, followed by a sharpening function to generate the sharpened label of $\boldsymbol{x}^\textit{u}$, yielding augmented data $(\boldsymbol{x}^\textit{u}, \boldsymbol{y}^\textit{u})$, \ie}
    \begin{equation}
        \begin{aligned}
           \hat{\boldsymbol{p}} = \frac{1}{N} &\sum_{i=1}^N \boldsymbol{p}_\textit{i} = \left[\hat{p}_1, \hat{p}_2, \cdots, \hat{p}_\textit{C}\right] \\
           y^\textit{u}_\textit{k} = \hat{p}_\textit{k}^{\frac{1}{T}} &/ \sum_{j=1}^C \hat{p}_\textit{j}^{\frac{1}{T}}, \quad 1 \leqslant k,j \leqslant C \\
            \boldsymbol{y}^\textit{u} &= \left[y^\textit{u}_\textit{1}, y^\textit{u}_\textit{2}, \cdots, y^\textit{u}_\textit{C}  \right] 
        \end{aligned}
    \end{equation}
    \emph{where $\hat{\boldsymbol{p}}$ is the average prediction distribution, $C$ is the number of classes, and $T$ is the temperature hyperparameter.}
\end{definition}
The process of sharpening-labeling is illustrated in Fig.~\ref{fig: sharpening-labeling}. Note that in practice, we usually choose temperature sharpening~\cite{DL-2015} as the sharpening function to reduce the entropy of the prediction distribution.
It is commonly used in conjunction with consistency regularization~\cite{NASA-2022,Graphmix-2021,GRAND-2020}.
Related work of sharpening-labeling is summarized in Table~\ref{tb: pseudo-labeling-strategy}.
GraphMix~\cite{Graphmix-2021} applies the average prediction on multiple random perturbations of an input unlabeled sample along with sharpening trick, further augments training data and improve prediction accuracy.
GRAND~\cite{GRAND-2020} utilizes sharpening-labeling to construct labels for unlabeled nodes based on the average prediction over multiple data augmentation, and further assists the implementation of consistency regularization.
NASA~\cite{NASA-2022} proposes a neighbor-constrained regularization to enforce the predictions of neighbors to be consistent with each other, in which the sharpening trick is used to generate label for the center node based on the average predictions of its neighbors.




% \subsubsection{Label Interpolation}
% \myTODO{===== TODO =====}

% \subsubsection{Summary}



% \begin{table*}
%     \renewcommand\arraystretch{1}
%     \centering
%     \caption{Summary of representative graph data augmentation works for graph learning. 
%     GDAug categories: 
%     FS: Feature Shuffling; 
%     FM: Feature Masking; 
%     ND: Node Dropping;
%     NI: Node Interpolation;
%     ER: Edge Rewiring;
%     SSa: Subgraph Sampling;
%     SSu: Subgraph Substitution;
%     GP: Graph Propagation;
%     GI: Graph Interpolation;
%     PL: Pseudo-Labeling;
%     SL: Sharpening-Labeling.}
%     \label{tb: all-work}
%     \resizebox{0.9\textwidth}{!}{%
%     \begin{tabular}{cccccl}
%     \toprule
%      Ref               & Model            & Publication   & Year & GDAug                                   & Code                                                                                                      \\
%      \midrule
%      \cite{DGI-2019}               & DGI              & ICLR          & 2019 & FS, ER                                  & https://github.com/PetarV-/DGI                                                                                                \\
%      \midrule
%      \cite{STDGI-2019}             & STDGI            & ICLR-workshop & 2019 & FS                                      & ---                                                                                                                          \\
%      \midrule
%      \cite{STABLE-2022}            & STABLE           & KDD           & 2022 & FS, ER                                  & ---                                                                                                                          \\
%      \midrule
%      \cite{HDMI-2021}              & HDMI             & WWW           & 2021 & FS                                      & https://github.com/baoyujing/HDMI                                                                                             \\
%      \midrule
%      \cite{HDGI-2020}              & HDGI             & AAAI-workshop & 2020 & FS                                      & https://github.com/YuxiangRen/Heterogeneous-Deep-Graph-Infomax                                                                \\
%      \midrule
%      \cite{HTC-arxiv}              & HTC              & Arxiv         & 2021 & FS                                      & ---                                                                                                                          \\
%      \midrule
%      \cite{Contrast-Reg-arxiv}     & Contrast-Reg     & Arxiv         & 2021 & FS                                      & ---                                                                                                                          \\
%      \midrule
%      \cite{FLAG-2022}              & FLAG             & CVPR          & 2022 & FM                                      & https://github.com/devnkong/FLAG                                                              \\
%      \midrule
%      \cite{Ethident-2022}          & Ethident         & IEEE-TIFS     & 2022 & FM, ND, ER, SSa                         & https://github.com/jjzhou012/Ethident                                                         \\
%      \midrule                       
%      \cite{SMICLR-2022}            & SMICLR           & JCIM          & 2022 & FM, ND, ER, SSa                         & https://github.com/CIDAG/SMICLR                                                               \\
%      \midrule                       
%      \cite{GraphCL-2020}           & GraphCL          & NeurIPS       & 2020 & FM, ND, ER, SSa                         & https://github.com/Shen-Lab/GraphCL                                                           \\
%      \midrule                       
%      \cite{JOAO-2021}              & JOAO             & ICML          & 2021 & FM, ND, ER, SSa                         & https://github.com/Shen-Lab/GraphCL\_Automated                                                \\
%      \midrule                       
%      \cite{AutoGRL-2021}           & AutoGRL          & IJCNN         & 2021 & FM, ND, ER, PL                          & https://github.com/JunweiSUN/AutoGRL                                                          \\
%      \midrule
%      \cite{LG2AR-arxiv}            & LG2AR            & Arxiv         & 2022 & FM, ND, ER, SSa                         & ---                                                                                                                          \\
%      \midrule
%      \cite{GRACE-2020}             & GRACE            & ICML-workshop & 2020 & FM, ER                                  & https://github.com/CRIPAC-DIG/GRACE                                                           \\
%      \midrule
%      \cite{GCA-2021}               & GCA              & WWW           & 2021 & FM, ER                                  & https://github.com/CRIPAC-DIG/GCA                                                             \\
%      \midrule
%      \cite{BGRL-2021}              & BGRL             & ICLR-workshop & 2021 & FM, ER                                  & https://github.com/nerdslab/bgrl                                                              \\
%      \midrule
%      \cite{BGRL-2022}              & BGRL             & ICLR          & 2022 & FM, ER                                  & https://github.com/Namkyeong/BGRL\_Pytorch                                                    \\
%      \midrule
%      \cite{GROC-2021}              & GROC             & WWW-workshop  & 2021 & FM, ER                                  & ---                                                                                                                          \\
%      \midrule
%      \cite{GBT-2022}               & GBT              & KBS           & 2022 & FM, ER                                  & https://github.com/pbielak/graph-barlow-twins                                                 \\
%      \midrule
%      \cite{NodeAug-2020}           & NodeAug          & KDD           & 2020 & FM, ER                                  & ---                                                                                                                          \\
%      \midrule
%      \cite{MeTA-2021}              & MeTA             & NeurIPS       & 2021 & FM, ER                                  & ---                                                                                                                          \\
%      \midrule
%      \cite{MERIT-2021}             & MERIT            & IJCAI         & 2021 & FM, ER, GP                              & https://github.com/GRAND-Lab/MERIT                                                            \\
%      \midrule
%      \cite{HeCo-2021}              & HeCo             & KDD           & 2021 & ND                                      & https://github.com/liun-online/HeCo                                                           \\
%      \midrule
%      \cite{GRAND-2020}             & GRAND            & NeurIPS       & 2020 & ND                                      & https://github.com/THUDM/GRAND                                                                \\
%      \midrule
%      \cite{MH-Aug-2021}            & MH-Aug           & NeurIPS       & 2021 & ND, ER                                  & https://github.com/hyeonzini/Metropolis-Hastings-Data-Augmentation-for-Graph-Neural-Networks  \\
%      \midrule
%      \cite{CSSL-2021}              & CSSL             & AAAI          & 2021 & ND, ER                                  & https://github.com/UCSD-AI4H/GraphSSL                                                         \\
%      \midrule
%      \cite{2branch-mixup}          & two-branch Mixup & WWW           & 2021 & NI, GI                                  & https://github.com/vanoracai/MixupForGraph                                                    \\
%      \midrule
%      \cite{Graphmix-2021}          & GraphMix         & AAAI          & 2021 & NI, SL                                  & https://github.com/vikasverma1077/GraphMix                                                    \\
%      \midrule
%      \cite{Graphsmote-2021}        & GraphSMOTE       & WSDM          & 2021 & NI                                      & https://github.com/TianxiangZhao/GraphSmote                                                   \\
%      \midrule
%      \cite{GraphENS-2021}          & GraphENS         & AAAI          & 2022 & NI                                      & https://github.com/JoonHyung-Park/GraphENS                                                    \\
%      \midrule
%      \cite{NodeAug-INS}            & NodeAug-INS      & CDS           & 2021 & NI                                      & ---                                                                                                                              \\
%      \midrule
%      \cite{GraphMixup-2022}        & GraphMixup       & ECML-PKDD     & 2021 & NI                                      & https://github.com/LirongWu/GraphMixup                                                        \\
%      \midrule
%      \cite{AugAN-arxiv}            & AugAN            & Arxiv         & 2022 & NI                                      & ---                                                                                                                          \\
%      \midrule
%      \cite{DropEdge-2020}          & DropEdge         & ICLR          & 2020 & ER                                      & https://github.com/DropEdge/DropEdge                                                                                          \\
%      \midrule
%      \cite{GAUG-2021}              & GAUG             & AAAI          & 2021 & ER                                      & https://github.com/zhao-tong/GAug                                                                                             \\
%      \midrule
%      \cite{RobustECD-2021}         & RobustECD        & IEEE-TKDE     & 2021 & ER                                      & https://github.com/jjzhou012/RobustECD                                                                                        \\
%      \midrule
%      \cite{Fairdrop-2021}          & FairDrop         & IEEE TAI      & 2021 & ER                                      & https://github.com/ispamm/FairDrop                                                                                            \\
%      \midrule
%      \cite{AD-GCL-2021}            & AD-GCL           & NeurIPS       & 2021 & ER                                      & https://github.com/susheels/adgcl                                                                                             \\
%      \midrule
%     %  \cite{AdaEdge}           & AdaEdge          & AAAI          & 2020 & ER                                      & https://github.com/victorchen96/MadGap                                                                                        \\
%     %  \midrule
%      \cite{PTDNet-2021}            & PTDNet           & WSDM          & 2021 & ER                                      & https://github.com/flyingdoog/PTDNet                                                                                          \\
%      \midrule
%      \cite{MEvolve-tnse}           & M-Evolve         & IEEE-TNSE     & 2020 & ER, PL                                  & ---                                                                                                                              \\
%      \midrule
%      \cite{SUGAR-2021}             & SUGAR            & WWW           & 2021 & SSa                                     & https://github.com/RingBDStack/SUGAR                                                          \\
%      \midrule
%      \cite{GCC-2020}               & GCC              & KDD           & 2020 & SSa                                     & https://github.com/THUDM/GCC                                                                  \\
%      \midrule
%      \cite{SUBG-CON}               & SUBG-COM         & ICDM          & 2020 & SSa                                     & https://github.com/yzjiao/Subg-Con                                                            \\
%      \midrule
%      \cite{Graphcrop-arxiv}        & GraphCrop        & Arxiv         & 2020 & SSa                                     & ---                                                                                                 \\
%      \midrule
%      \cite{InfoGraph-2020}         & InfoGraph        & ICLR          & 2020 & SSa                                     & https://github.com/fanyun-sun/InfoGraph                                                       \\
%      \midrule
%      \cite{EGI-2021}               & EGI              & NeurIPS       & 2021 & SSa                                     & https://github.com/GentleZhu/EGI                                                              \\
%      \midrule
%      \cite{NeuralSparse-2020}      & NeuralSparse     & ICML          & 2020 & SSa                                     & https://github.com/flyingdoog/PTDNet/tree/main/NeuralSparse                                   \\
%      \midrule
%      \cite{MVGRL-2020}             & MVGRL            & ICML          & 2020 & SSa, GP                                 & https://github.com/kavehhassani/mvgrl                                                                                         \\
%      \midrule
%      \cite{SubMix-2022}            & SubMix           & WWW           & 2022 & SSu                                     & https://github.com/snudatalab/GraphAug                                                                                        \\
%      \midrule
%      \cite{Graph-Transplant-2022}  & Graph Transplant & AAAI          & 2022 & SSu                                     & ---                                                                                                                          \\
%      \midrule
%      \cite{MoCL-2021}              & MoCL             & KDD           & 2021 & SSu                                     & https://github.com/illidanlab/MoCL-DK                                                         \\
%      \midrule
%      \cite{GREA-2022}              & GREA             & KDD           & 2022 & SSu                                     & https://github.com/liugangcode/GREA                                                           \\
%      \midrule
%      \cite{SelfGNN-2021}           & SelfGNN          & WWW-workshop  & 2021 & GP                                      & https://github.com/zekarias-tilahun/SelfGNN                                                                                   \\
%      \midrule
%      \cite{MV-GCN-2021}            & MV-GCN           & CIKM          & 2021 & GP                                      & ---                                                                                                                              \\
%      \midrule
%      \cite{GDC-2019}               & GDC              & NeurIPS       & 2019 & GP                                      & https://github.com/gasteigerjo/gdc                                                                                            \\
%      \midrule
%      \cite{G-Mixup-2022}           & G-mixup          & ICML          & 2022 & GI                                      & https://github.com/ahxt/g-mixup                                                               \\
%      \midrule
%      \cite{ifmixup-arxiv}          & ifMixup          & arxiv         & 2021 & GI                                      & ---                                                                                                                              \\
%      \midrule
%      \cite{NASA-2022}              & NASA             & AAAI          & 2022 & SL                                      & https://github.com/BUPT-GAMMA/NASA                                                                                            \\
%      \midrule
%      \cite{CGCN-2020}              & CGCN             & AAAI          & 2020 & PL                                      & ---                                                                                                                          \\
%      \midrule
%      \cite{M3S-2020}               & M3S              & AAAI          & 2020 & PL                                      & https://github.com/Junseok0207/M3S\_Pytorch                                                                                   \\
%      \midrule
%      \cite{NRGNN-2021}             & NRGNN            & KDD           & 2021 & PL                                      & https://github.com/EnyanDai/NRGNN                                                                                             \\
%     \bottomrule              
% \end{tabular}}
% \end{table*}
























% \begin{algorithm}[H]
%     \caption{The HALO Algorithm}
%     \KwData{$G=(V,E)$, $r_B$}
%     \KwResult{$Boxes$, $N_B$}
%     \tcc{box sampling stage}
%     Initialize sampling boxes $B=\emptyset$, uncovered nodes $U=V$, seed nodes $C=\emptyset$\;
%     \While{$U\neq \emptyset$}{
%       $box=\emptyset$\;
%       calculate excluded mass $em_i$ for the current non-seed nodes \;
%     %   $p= \underset{i\in U}{\arg\max} \ em_i$ \textcolor{blue}{\Comment{get node that maximizes excluded mass}}\; 
%       $p= {\arg\max}_{i\in U} \ em_i$ \textcolor{blue}{\Comment{get node that maximizes excluded mass}}\;  
%       $C=C \cup \{p\}$ \;
%       $box = box \cup \{p\}$ \;
%       $box = box \cup \{i \mid i \in U \land d_{ip} \le r_B \}$\textcolor{blue}{\Comment{get nodes with distance no more that $r_B$ from $p$}} \;
%       $U=U\setminus box$\;
%       $B = B\cup box$\;
%     }


%     %   \Repeat{this end condition}{
%     %     do these things \textcolor{blue}{\Comment{{this is a comment}}} \;
%     %   }
%     %   \eIf{understand}{
%     %     go to next section\;
%     %     current section becomes this one\;
%     %   }{
%     %     go back to the beginning of current section\;
%     %   }
%     %   \Do{this end condition}{
%     %     do these things\;
%     %   }
%     % }
    
% \end{algorithm}


% \begin{algorithm}[H]
%     \SetNoFillComment
%     \caption{The HALO Algorithm, Step 1: Box sampling stage}
%     % \KwData{$G=(V,E)$, $r_B$}
%     \KwIn{graph $G=(V,E)$, $r_B$}
%     \KwOut{sampled boxes $B$}
%     % step 1-1
%     \tcc{Forward rule box sampling}
%     Initialize sampling boxes $B=\emptyset$, uncovered nodes $U=V$, seed nodes $C=\emptyset$\;
%     \While{$U\neq \emptyset$}{
%         $box=\emptyset$\;
%         Calculate excluded mass $em_i$ for the current non-seed nodes \;
%         %   $p= \underset{i\in U}{\arg\max} \ em_i$ \textcolor{blue}{\Comment{get node that maximizes excluded mass}}\; 
%         $p= {\arg\max}_{i\in U} \ em_i$   \tcp*{get node that maximizes excluded mass}   
%         $C=C \cup \{p\}$ \;
%         $box = box \cup \{p\}$ \;
%         $box = box \cup \{i \mid \forall i \in U \land l_{ip} \le r_B \}$    \tcp*{nodes with distance no more that $r_B$ from $p$}
%         $U=U\setminus box$\;
%         $B = B\cup \{box\}$\;
%     }
%     % step 1-2
%     \tcc{Setp 1-2: Reverse rule box sampling}
%     Initialize $l_B = 2r_B + 1$, uncovered nodes $U=V$\;
%     Calculate degree value $d_i$ for each node\;
%     \While{$U \neq \emptyset$}{
%         $box=\emptyset$\;
%         $p= {\arg\min}_{i\in U} \ d_i$   \tcp*{get node with minimal degree value}  
%         $box = box \cup \{p\}$ \;
%         $R=\{i \mid \forall i \in U \land l_{ip} < l_B \}$ \tcp*{nodes with distance less that $l_B$ from $p$}
%         \While{$R \neq \emptyset$}{
%             $N=U \cap R$\;
%             \If{$N \neq \emptyset$}{
%                 $n \leftarrow \operatorname{RandomSampling}(N)$ \tcp*{randomly sample a node from $N$}
%             }
%             \Else{
%                 $n \leftarrow \operatorname{RandomSampling}(R)$ \tcp*{randomly sample a node from $R$}
%             }
%             $box = box \cup \{n\}$\;
%             $R = R \setminus \{n\}$\;
%             $K=\{i \mid \forall i \in U \land l_{in} < l_B \}$ \tcp*{nodes with distance less that $l_B$ from $n$}
%             $R=R\cap K$\;
%         }
%         $U=U\setminus box$\;
%         $B = B\cup \{box\}$\;
%     }
%     \textbf{Return:} sampled boxes $B$
% \end{algorithm}



==> 6-metric_copy.tex <==
\section{Evaluation Metrics and Design Guidelines}\label{sec: metrics}
In this section, we summarize existing metrics and guidelines for evaluating or designing \gda~ techniques.
We first introduce several evaluation metrics that are commonly used in graph analysis tasks, and then introduce some new metrics and guidelines specifically designed for \gda.

\subsection{Common Metrics}
% Since \gda~ is an auxiliary technique, existing studies usually indirectly reflect the effectiveness of \gda~ by evaluating the performance of downstream tasks.

Since \gda~ is an auxiliary technique, existing studies often measures its effectiveness by evaluating the performance improvements in downstream tasks achieved with its assistance.
For classification tasks like node classification~\cite{MeTA-2021,NodeAug-2020} and graph classification~\cite{MEvolve-cikm,Ethident-2022}, it is common to use accuracy-based metrics such as \textbf{Accuracy}, \textbf{Precision}, \textbf{F1 score}, \textbf{Area Under Curve (AUC)} and \textbf{Average Precision (AP)} for reflecting the classification performance from different perspectives.
For graph representation learning~\cite{InfoGraph-2020,GCA-2021,SUBG-CON,MVGRL-2020}, the learned embeddings will be fed into the downstream classifiers or clustering algorithms, and evaluated via accuracy-based metrics as mentioned above, or clustering-based metrics such as \textbf{Normalized Mutual Information (MNI)} and \textbf{Adjusted Rand Index (ARI)}.
Additionally, several works apply \gda~ in pre-training task~\cite{GCC-2020} or recommendation~\cite{SGL-2021}, followed by evaluation with ranking-based metrics like \textbf{HITS@$k$}.

\subsection{Specific Metrics and Design Guidelines}
Besides the common metrics above, several special metrics and guidelines have been proposed to evaluate the performance of \gda~ or guide the design of \gda.
Here we present the detailed definitions and descriptions of them.

% \begin{itemize}
%     \item \textbf{Change Ratio} (\cite{MEvolve-tnse,MH-Aug-2021,SubMix-2022}). This metric is mainly used to measure the degree of modification of graph structure and features during manipulation-based augmentation (as mentioned in Sec.~\ref{sec: taxonomy-mechanism}). It describes the modification ratio of nodes, edges, and features before and after augmentation. Formally, for the original graph $G=(\mathcal{V}, \mathcal{E}, \boldsymbol{X})$ and the augmented graph $\hat{G}=(\hat{\mathcal{V}}, \hat{\mathcal{E}}, \hat{\boldsymbol{X}})$, the 
% \end{itemize}

\subsubsection{Change Ratio}
This metric is mainly used to measure the degree of modification of graph structure and features during manipulation-based augmentation (as mentioned in Sec.~\ref{sec: taxonomy-mechanism}). Formally, we have the following generalized definition of change ratio:
\begin{definition}
    \textbf{Change Ratio}.
    \emph{Given a graph $G=(\mathcal{V}, \mathcal{E}, \boldsymbol{X})$ and its augmentation $\hat{G}=(\hat{\mathcal{V}}, \hat{\mathcal{E}}, \hat{\boldsymbol{X}})$, the change ratio of $G$ to $\hat{G}$ is measured by the number of modified nodes (or edges, features) divided by the number of original nodes (or edges, features), \ie}
    \begin{equation}
        \begin{aligned}
            &M_{\Delta \mathcal{V}} = (|\mathcal{V} - \hat{\mathcal{V}}| + |\hat{\mathcal{V}} - \mathcal{V}|) / |\mathcal{V}| \\
            &M_{\Delta \mathcal{E}} = (|\mathcal{E} - \hat{\mathcal{E}}| + |\hat{\mathcal{E}} - \mathcal{E}|) / |\mathcal{E}| \\
            &M_{\Delta \boldsymbol{X}} = \Vert \hat{\boldsymbol{x}} - \boldsymbol{x}\Vert_0 / F
        \end{aligned}
    \end{equation}
    % \begin{equation}
    %     \begin{aligned}
    %         &\Delta \mathcal{V} = \frac{|\mathcal{V} - \hat{\mathcal{V}}| + |\hat{\mathcal{V}} - \mathcal{V}|}{|\mathcal{V}|}  \\
    %         &\Delta \mathcal{E} = \frac{|\mathcal{E} - \hat{\mathcal{E}}| + |\hat{\mathcal{E}} - \mathcal{E}|}{|\mathcal{E}|}  \\
    %         &\Delta \boldsymbol{X} = \frac{||\hat{\boldsymbol{x}} - \boldsymbol{x}||_0}{F}
    %     \end{aligned}
    % \end{equation}
   \emph{where $F$ is the dimension of feature vector, and $\Vert \cdot\Vert_0$ is the zero norm.}
\end{definition}
It describes the modification ratio of nodes, edges, or features before and after augmentations like node dropping~\cite{MH-Aug-2021}, edge rewiring~\cite{MEvolve-tnse,MH-Aug-2021} and feature masking~\cite{GRACE-2020}, and can also be regarded as a probability hyperparameter to guide augmentations.
For example, in global uniform feature masking, the probability $p^\textit{m}_\textit{ij}$ of masking an attribute is equivalent to $M_{\Delta \boldsymbol{X}}$.
% Furthermore, this metric can also be used as a constraint when designing augmentation strategies.
% For example, M-Evolve~\cite{MEvolve-tnse} follows the structure-preserving principle, which requires that the augmentation strategy does not change the number of edges in the target graph, \ie setting $M_{\Delta \mathcal{E}}=0$.
% SubMix~\cite{SubMix-2022} proposes five desired properties for effective graph augmentations, including size preservation, which states that augmentation should satisfy an unbiased change of graph size, \ie equivalent to $M_{\Delta \mathcal{V}}=0$ and $M_{\Delta \mathcal{E}}=0$.


\subsubsection{Tradeoff in \gda~ via Consistency and Diversity}
NASA~\cite{NASA-2022} proposes two metrics, \ie consistency and diversity, to measure the correctness and generalization of \gda, respectively.
We present the definition of them as follows:
\begin{definition}
    \textbf{Consistency vs. Diversity}.
    \emph{For two models $f_\theta$ and $\hat{f}_\theta$, which are trained from the training set $\mathcal{D}_\textit{train}$ and its augmentation $\hat{\mathcal{D}}_\textit{train}$ respectively, the consistency can be represented by the accuracy of augmented model $\hat{f}_\theta$ on validation set $\mathcal{D}_\textit{val}$, \ie}
    \begin{equation}
        M_\textit{c} = \operatorname{Acc}\left(\hat{f}_\theta \left(\mathcal{D}_\textit{val}\right), \mathcal{Y}_\textit{val}\right)
    \end{equation}
    \emph{where $\mathcal{Y}_\textit{val}$ is the labels of validation set.
    The diversity can be represented by the prediction difference between augmented model $\hat{f}_\theta$ and original model $f_\theta$ on validation set, \ie}
    \begin{equation}
        M_\textit{d} = \Vert \hat{f}_\theta \left(\mathcal{D}_\textit{val}\right) - f_\theta \left(\mathcal{D}_\textit{val}\right) \Vert^2_\textit{F}
    \end{equation}
    \emph{where $\Vert \cdot\Vert_\textit{F}$ is the Frobenius norm.}
\end{definition}
% Consistency and diversity are used to measure the correctness and generalization of augmentations, respectively.
Specifically, a lower consistency indicates that the augmentation hurts the original data distribution, but a higher consistency may not contribute well to the generalization of the model while maintaining correctness.
On the other hand, a lower diversity indicates that the augmentation contributes little to the generalization of the model, while a higher diversity cannot ensure the correctness of the augmentation.
Neither metric alone can fully evaluate the quality of augmentation. 
Therefore, NASA combines these two metrics to trade off the design of \gda, expecting to achieve augmentation with better correctness and generalization, improve the performance of augmented models, and build generalized decision boundaries.


\subsubsection{Tradeoff in \gda~ via Affinity and Diversity}
\citet{trivedi2022augmentations} state that augmentation should generate samples that are close enough to the original data to share task-relevant semantics, while being sufficiently different to prevent trivially similar samples.
They utilize two metrics to quantify the above tradeoff, affinity and diversity, as proposed in~\cite{gontijo2020tradeoffs}.
We present the definition of them as follows:
\begin{definition}
    \textbf{Affinity vs. Diversity}.
    \emph{For a model $f_\theta$ trained from the training set $\mathcal{D}_\textit{train}$, the affinity can be measured by the accuracy on augmented validation set $\hat{\mathcal{D}}_\textit{val}$ divided by the accuracy on the original validation set $\mathcal{D}_\textit{val}$, \ie}
    \begin{equation}
        M_\textit{A} = \frac{\operatorname{Acc}(f_\theta (\hat{\mathcal{D}}_\textit{val}), \mathcal{Y}_\textit{val})}{\operatorname{Acc}(f_\theta (\mathcal{D}_\textit{val}), \mathcal{Y}_\textit{val})}
    \end{equation}
    \emph{where $\mathcal{Y}_\textit{val}$ is the labels of validation set.
    And the diversity can be measured by the ratio of the final training loss on the augmented training set $\hat{\mathcal{D}}_\textit{train}$, relative to the final training loss on the original training set $\mathcal{D}_\textit{train}$, \ie}
    \begin{equation}
        M_\textit{D} = \mathbb{E}[\hat{\mathcal{L}}_\textit{train}] / \mathbb{E}[\mathcal{L}_\textit{train}]
    \end{equation}
\end{definition}
Specifically, the affinity metric is used to quantify the distribution shift of the augmented data compared to the original data, with a lower affinity indicating that the augmented data is out-of-distribution for the model.
On the other hand, the diversity metric quantifies how difficult it is for a model to learn from augmented data rather than original data.


\subsubsection{Preserving Connectivity}
Several works~\cite{MEvolve-tnse,SubMix-2022} state that the connectivity information of a graph before and after augmentation should not be changed, as defined below.
\begin{definition}
    \textbf{Preserving Connectivity}.
    \emph{For a graph $G$ and its augmentation $\hat{G}$, $\hat{G}$ should follow the connectivity information of $G$, \ie $\hat{G}$ should be connected if and only if $G$ is connected.}
\end{definition}

% \subsubsection{Consistency}

% \subsubsection{Diversity}
